Impact of demand growth on decarbonizing India's electricity sector and the role for energy storage

Global energy sector decarbonization efforts are contingent on technology choices for energy production and end-use in emerging markets such as India, where air conditioning is expected to be a major driver for electricity demand growth. Here, we use an integrated demand-supply framework to quantify the impacts of demand growth and temporal patterns on long-term electricity system evolution. Under projected renewables and Li-ion storage cost declines, our supply-demand modeling points to renewables contributing substantially (46-67%) to meet annual electricity demand in India by 2030. However, without appropriate policy measures to phase out existing coal generation, even such rapid adoption of renewable energy coupled with one or more technological levers such as low-cost energy storage and demand-side measures such as setting aggressive AC efficiency standards and deploying distribution level storage, are insufficient to reduce annual CO2 emissions in 2050 vs. 2020 because of the relatively higher growth rate of projected electricity demand over this period.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
